On the gravitization of quantum mechanics and wave function reduction in Bohmian quantum mechanics

The main topic of this paper is using Einstein's equivalence principle in the description of the gravity-induced wave function reduction in the framework of Bohmian causal quantum theory. However, such concept has been introduced and explored by Penrose for the standard quantum mechanics, but the capabilities of Bohmian quantum mechanics makes it possible to get some of results more clearly. In this regard, the critical mass for transition from the quantum world to the classical world, the reduction time of the wave function and the temperature that corresponds to the Unruh temperature will be obtained by applying Einstein's equivalence principle for the quantum motion of particle.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


